EAM: Enhancing Anything with Diffusion Transformers for Blind Super-Resolution

Utilizing pre-trained Text-to-Image (T2I) diffusion models to guide Blind Super-Resolution (BSR) has become a predominant approach in the field. While T2I models have traditionally relied on U-Net architectures, recent advancements have demonstrated that Diffusion Transformers (DiT) achieve significantly higher performance in this domain. In this work, we introduce Enhancing Anything Model (EAM), a novel BSR method that leverages DiT and outperforms previous U-Net-based approaches. We introduce a novel block, $\Psi$-DiT, which effectively guides the DiT to enhance image restoration. This block employs a low-resolution latent as a separable flow injection control, forming a triple-flow architecture that effectively leverages the prior knowledge embedded in the pre-trained DiT. To fully exploit the prior guidance capabilities of T2I models and enhance their generalization in BSR, we introduce a progressive Masked Image Modeling strategy, which also reduces training costs. Additionally, we propose a subject-aware prompt generation strategy that employs a robust multi-modal model in an in-context learning framework. This strategy automatically identifies key image areas, provides detailed descriptions, and optimizes the utilization of T2I diffusion priors. Our experiments demonstrate that EAM achieves state-of-the-art results across multiple datasets, outperforming existing methods in both quantitative metrics and visual quality.

==> figures/ab1.tex <==
\begin{figure}[t]
 \centering
 \scalebox{0.45}{
 \includegraphics[width=\textwidth]{figures/abaltion1.pdf}
 \vspace{-0.5cm}
 }
 \caption{Restoration results using different architecture, from the left to the right: the whole LR input, the cropping input region, the corresponding restoration of DiT-controlnet, the result of EAM (Ours).}
 \vspace{-10pt}
 \label{ab1}
\end{figure}

==> figures/ab2.tex <==
\begin{figure}[t]
 \centering
 \scalebox{0.45}{
 \includegraphics[width=\textwidth]{figures/abaltion2.pdf}
 \vspace{-0.5cm}
 }
 \caption{Restoration results of model using PMS or not. from the left to the right: the whole LR input, the cropping input region, model results trained without PMS, model results trained with PMS.}
 \vspace{-10pt}
 \label{fig:ab2}
\end{figure}

==> figures/fDIT_note.tex <==
\begin{figure}[t]
 \centering
 \scalebox{0.6}{
 \includegraphics[width=\textwidth]{figures/fDIT_plus.pdf}
 \vspace{-0.5cm}
 }
 \caption{Detail of $\Psi$-DIT: On the left, we have the pre-trained MMDIT architecture, which remains frozen to preserve its learned patterns. On the right, we introduce our novel trainable module, the Separable Stream Control Module (SSCM), designed to enhance the model's adaptability and performance.}
 \vspace{-10pt}
 \label{content}
\end{figure}

==> figures/frame_work.tex <==
\begin{figure*}[t]
 \centering
 \scalebox{1}{
 \includegraphics[width=\textwidth]{figures/main_schedule_new.pdf}
 \vspace{-0.5cm}
 }
 \caption{This figure briefly demonstrate the training workflow of our proposed EAM method.}
 % \vspace{1.5cm}
 \label{framework}
\end{figure*}


==> figures/maincompare.tex <==
\begin{figure*}[]
	%\newlength-4mm
	%\setlength{-4mm}{-0.4cm}
	\scriptsize
	\centering
    \vspace{-4mm}
    \resizebox{\textwidth}{!}{
	\begin{tabular}{l}
		\hspace{-0.42cm}
		\begin{adjustbox}{valign=t}
  \scalebox{1}{
			\begin{tabular}{c}
				\includegraphics[width=0.409\textwidth]{{figures/cmp0/LR.png}}
                \\
                \method{} LR
				\hspace{-10mm}
			\end{tabular}}
		\end{adjustbox}
		\hspace{-5mm}
		\begin{adjustbox}{valign=t}
			\begin{tabular}{ccc}
				\includegraphics[width=0.19\textwidth]{figures/cmp0/stablesr.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp0/diffbir.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp0/pasd.png} \hspace{-4.5mm} 
				\\
				StableSR\cite{wang2023exploiting}  \hspace{-2mm} &
				DiffBIR\cite{lin2023diffbir} \hspace{-3.5mm} &
			    PASD\cite{yang2023pixel}	\hspace{-3.5mm}
				\\
				\includegraphics[width=0.19\textwidth]{figures/cmp0/seesr.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp0/supir.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp0/eam.png} \hspace{-4.5mm}
				\\ 
				SeeSR \hspace{-3.5mm} &
				SUPIR \hspace{-3.5mm} &
				\method{} EAM (ours) \hspace{-3.5mm}
			\end{tabular}
		\end{adjustbox}
		\hspace{-2mm}
        \\
		\hspace{-0.42cm}
		\begin{adjustbox}{valign=t}
			\begin{tabular}{c}
				\includegraphics[width=0.409\textwidth]{{figures/cmp1/LR.png}}
                \\
                \method{} LR
				\hspace{-10mm}
			\end{tabular}
		\end{adjustbox}
		\hspace{-5mm}
		\begin{adjustbox}{valign=t}
			\begin{tabular}{ccc}
				\includegraphics[width=0.19\textwidth]{figures/cmp1/stablesr.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp1/diffbir.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp1/pasd.png} \hspace{-4.5mm} 
				\\
				StableSR\cite{wang2023exploiting}  \hspace{-2mm} &
				DiffBIR\cite{lin2023diffbir} \hspace{-3.5mm} &
			    PASD\cite{yang2023pixel}	\hspace{-3.5mm}
				\\
				\includegraphics[width=0.19\textwidth]{figures/cmp1/seesr.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp1/supir.png} \hspace{-4.5mm} &
				\includegraphics[width=0.19\textwidth]{figures/cmp1/eam.png} \hspace{-4.5mm}
				\\ 
				SeeSR \hspace{-3.5mm} &
				SUPIR \hspace{-3.5mm} &
				\method{} EAM (ours) \hspace{-3.5mm}
			\end{tabular}
		\end{adjustbox}
		\hspace{-2mm}
	\end{tabular}
    % \hspace{-8mm}
    \vspace{-4mm}
	\caption{Qualitative comparison with different methods on DIV2K. Our EAM can restore the texture and details. Other methods recover with unpleasing details or irregular faces.}
    \label{fig1:main_visual}
	\vspace{-4mm}
\end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> figures/real_compare.tex <==
\begin{figure*}[t]
 \centering
 \scalebox{1}{
 \includegraphics[width=\textwidth]{figures/compr_q.pdf}
 \vspace{-0.5cm}
 }
 \caption{Qualitative comparison with different methods on real world inputs. Our EAM can restore the inputs with more realistic details.}
 \vspace{-10pt}
 \label{RealWorld Compare}
\end{figure*}

==> figures/title.tex <==
\twocolumn[{
	\renewcommand\twocolumn[1][]{#1}
	\maketitle
	\thispagestyle{empty}
	\vspace{-30pt}
	\begin{center}
		\includegraphics[width=\linewidth]{figures/title.pdf}
		\vspace{-18pt}
            \captionof{figure}{
                Our EAM model can enhance the real-world low-quality images with realistic details.
            }
		\label{fig:first}
		\vspace{5pt}
	\end{center}
}]

==> sec/0_abstract.tex <==
\begin{abstract}
% A lot of work has been done to supersect blind images by using pre-trained diffusion to generate priors. DiT is a new and widely used diffusion architecture for SOTA. Despite its simpler architecture and stronger scale-up features, it has yet to prove its potential in blind image super-resolution tasks. In this work, we design a new blind overscore framework EAM based on the powerful pre-trained DiT graph model, which for the first time outperforms all previous blind overscore work based on unet diffusion. Through extensive research, we find that the original controlnet fine-tuning framework limits the ability of pre-trained DiT generation, so we propose a new $\Psi$-DiT fine-tuning framework. The LR latent is used as a separable flow injection control to form a tributary architecture, which can stimulate the priori of the pre-trained DiT model. In addition, in order to further improve the generalization ability of EAM to LR degradation and reduce the training cost, we introduce the training strategy of mask, which is proved to be effective by many experiments. Finally, we found that although the state-of-the-art VLM model was able to describe the output of high-definition pictures in detail, the description of low-quality pictures did not meet our requirements. We use the ICL technique to guide the VLM model to ignore the blind degradation of the input of low-quality images and output more imaginative text descriptions. Our final model achieves SOTA results on both synthetic and real-world test sets.
Utilizing pre-trained Text-to-Image (T2I) diffusion models to guide Blind Super-Resolution (BSR) has become a predominant approach in the field.
While T2I models have traditionally relied on U-Net architectures, recent advancements have demonstrated that Diffusion Transformers (DiT) achieve significantly higher performance in this domain.
In this work, we introduce Enhancing Anything Model (EAM), a novel BSR method that leverages DiT and outperforms previous U-Net-based approaches.
We introduce a novel block, $\Psi$-DiT, which effectively guides the DiT to enhance image restoration.
This block employs a low-resolution latent as a separable flow injection control, forming a three-branch architecture that effectively leverages the prior knowledge embedded in the pre-trained DiT.
To fully exploit the prior guidance capabilities of T2I models and enhance their generalization in BSR, we introduce a progressive Masked Image Modeling strategy, which also reduces training costs.
Additionally, we propose a subject-aware prompt generation strategy that employs a robust multi-modal model in an in-context learning framework. This strategy automatically identifies key image areas, provides detailed descriptions, and optimizes the utilization of T2I diffusion priors.
Our experiments demonstrate that EAM achieves state-of-the-art results across multiple datasets, outperforming existing methods in both quantitative metrics and visual quality.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Blind Super-Resolution (BSR) is a fundamental and crucial task in low-level computer vision, aiming to reconstruct high-resolution (HR) images from low-resolution (LR) images without relying on prior knowledge of the image degradation process. Compared to traditional super-resolution tasks, BSR holds greater practical significance, as the degradation process of images is often unknown or complex in real-world application scenarios.

With the rapid advancement of deep learning, training effective neural networks has emerged as the dominant approach for super-resolution (SR) tasks. In the early stages, pioneering works~\cite{dong2015imagesuperresolutionusingdeep,kim2016accurateimagesuperresolutionusing,lim2017enhanceddeepresidualnetworks,Hui_2019} utilized traditional convolutional neural networks (CNNs)~\cite{oshea2015introductionconvolutionalneuralnetworks} to predict SR images. However, the quality of the generated SR images often fell short due to the limited capacity of these networks, resulting in reconstructed images that lacked fine details and exhibited noticeable artifacts.
Subsequently, Generative Adversarial Networks (GANs)~\cite{goodfellow2014generative} were introduced to address these limitations. Notably, classical SR networks such as~\cite{ledig2017photorealisticsingleimagesuperresolution, zhang2021blind, wang2021real} leveraged the adversarial training paradigm of GANs to enhance the realism and quality of generated SR images. Despite these improvements, the inherent limitations of GAN-based methods, such as mode collapse and training instability, still posed challenges in consistently producing high-fidelity SR images with rich details.

In recent years, generative modeling has witnessed remarkable progress, especially in the realm of text-to-image generation. Among these innovations, diffusion models have garnered significant attention for their exceptional ability to generate high-quality, photorealistic images.
A notable milestone in this development is Stable Diffusion and its successors, which have significantly advanced text-to-image synthesis~\cite{rombach2022highresolutionimagesynthesislatent, podell2023sdxlimprovinglatentdiffusion}.These models are primarily based on the U-Net architecture~\cite{ronneberger2015unetconvolutionalnetworksbiomedical}, a widely-used framework for tasks such as segmentation and denoising.
Moreover, there has been a growing trend toward integrating Diffusion Transformers (DiTs) into these models~\cite{peebles2023scalablediffusionmodelstransformers}. Prominent examples include~\cite{esser2024scalingrectifiedflowtransformers,li2024hunyuanditpowerfulmultiresolutiondiffusion}. 
These models leverage attention mechanisms to handle long-range dependencies and complex data relationships, thereby enhancing the generative capabilities of diffusion models. The adoption of the DiTs architecture has unveiled extraordinary potential, continually pushing the boundaries of text-to-image generation.

Driven by the remarkable achievements of diffusion models, diffusion-based methods have been increasingly adopted in the super-resolution (SR) field, with notable examples including~\cite{wang2023exploiting,lin2023diffbir, yang2023pixel, wu2024seesrsemanticsawarerealworldimage, yu2024scalingexcellencepracticingmodel}. These methods commonly adhere to the ControlNet paradigm~\cite{zhang2023addingconditionalcontroltexttoimage}, a controllable diffusion model that introduces a separate branch alongside the basic diffusion model. This design enables customization of target high-resolution (HR) images by leveraging processed low-resolution (LR) latent representations and associated semantic prompts. 

However, our experiments reveal that this paradigm limits the generative capacity of the base model, as the control branch is isolated from the main branch. Given the emergence of Diffusion Transformers (DiTs) as potent diffusion networks, developing a DiT-based SR model is essential. 
Predictably, the limitations of ControlNet will become a bottleneck for achieving excellent SR performance in DiT-based SR networks.

To address this situation, we propose Enhancing Anything Model (EAM), a unique DiT-based architecture for blind image SR. Based on a pre-trained text-to-image DiT, we construct a triple-flow DiT block, termed $\Psi$-DiT, in which the noisy latents interact with both text embeddings and LR latents through attention operations. Our ablation experiments show that the modified blocks outperform traditional ControlNet. Additionally, we employ a new training strategy to enhance the generative power and robustness of the entire model. For semantic prompts, we adopt the state-of-the-art vision-language model (VLM) Mini-CPM~\cite{hu2024minicpmunveilingpotentialsmall} with a context learning approach to provide semantic information, which improves the SR performance. Extensive experiments demonstrate that our model achieves excellent pixel-level SR performance and outperforms existing SR methods on realistic test datasets.

In summary, our main contributions are:
\begin{itemize}
\item We propose EAM, a novel framework for applying DiT models to image SR tasks.
\item We design a novel triple-flow DiT architecture that enhances the base model's generative capacity by eliminating the control branch isolation inherent in the ControlNet paradigm, thereby improving output expressiveness and fidelity.
\item We introduce a Progressive MIM strategy in the control branch of the triple-flow block to maximize the generative potential of diffusion models while improving robustness.
\item We improve subject-aware prompt generation through multi-modal modeling and in-context learning.
\item We demonstrate that EAM achieves superior perceptual quality and improved generation effects for blind image super-resolution compared to existing methods, as shown through both quantitative and qualitative evaluations.
\end{itemize}




==> sec/1_intro_ref.tex <==
\section{Introduction Ref}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}
\paragraph{Traditional SR Modeling}
In recent years, the field of image Super-Resolution (SR) has progressed rapidly, moving from traditional interpolation techniques to deep learning-based approaches that deliver state-of-the-art results. SRCNN~\cite{dong2015imagesuperresolutionusingdeep} is the first work using CNNs to build the SR network. Notably,~\cite{kim2016accurateimagesuperresolutionusing,lim2017enhanceddeepresidualnetworks}achieved significant performance gains by using a much deeper network and taking more delicate training strategy. However, these SR models mostly produce rough images, as they are trained under simple degradation settings. 
To handle more complex SR tasks, GAN-based networks rise to the occasion. The first major GAN-based SR model is SRGAN~\cite{ledig2017photorealisticsingleimagesuperresolution}, introduced the use of an adversarial loss alongside a perceptual loss that operates in the feature space of a pretrained deep network. The subsequent models, BSRGAN~\cite{zhang2021blind}, further introduces a more powerful network focusing on blind SR. Another important development is Real-ESRGAN~\cite{wang2021real},which aims to handle real-world images degraded by complex factors.

\paragraph{Text-to-Image Diffusion Modeling}
In the field of generative modeling, the rapid development of diffusion models has gained a great deal of attention. Initially, diffusion models like DDPM~\cite{ho2020denoising} were used in probabilistic modeling, where they simulate the process of adding noise to data and then learn to reverse this process, progressively recovering data from noisy inputs. Over recent years, Stable Diffusion and its derivative works~\cite{rombach2022highresolutionimagesynthesislatent, podell2023sdxlimprovinglatentdiffusion} have shown impressive results in generating high-quality images, surpassing traditional models due to their stability and ability to generate detailed, realistic outputs. Furthermore, Diffusion Transformer (DiT)~\cite{peebles2023scalablediffusionmodelstransformers} exhibits plenty of generation potential on various tasks and outperforms the UNet-based architecture used by Stable Diffusion. It has been successfully applied in ~\cite{esser2024scalingrectifiedflowtransformers, li2024hunyuanditpowerfulmultiresolutiondiffusion}.
In addition, ControlNet~\cite{zhang2023addingconditionalcontroltexttoimage} and its similar works IP-Adapter~\cite{ye2023ipadaptertextcompatibleimage}, ControlNet++~\cite{li2024controlnetimprovingconditionalcontrols}, ControlNeXt~\cite{peng2024controlnextpowerfulefficientcontrol} provide diverse kinds of controllable diffusion architecture for more flexible customization of text-to-image, by leveraging a replicated portion of the pretrained diffusion model.

\paragraph{Diffusion-based SR Modeling}
The astonishing performances of text-to-image diffusion models stimulate the growth of diffusion-based SR modeling, among which ~\cite{wang2023exploiting,lin2023diffbir, yang2023pixel, wu2024seesrsemanticsawarerealworldimage, yu2024scalingexcellencepracticingmodel} are the representative examples. The aforementioned methods commonly use the paradigm of ControlNet-based SR, which creates an extra branch of the base diffusion model, in order to inject processed LR latent, semantic-aware prompts and other helpful knowledge for SR. For instance, PASD~\cite{yang2023pixel} uses LRs that processed by SwinIR~\cite{liang2021swinirimagerestorationusing} as the input of the ControlNet, and injects captions or detection results into the main branch. SeeSR~\cite{wu2024seesrsemanticsawarerealworldimage} uses DAPE to get representation embeddings and tags of LRs, then inject them into the ControlNet and the text encoder respectively. SUPIR~\cite{yu2024scalingexcellencepracticingmodel} significantly scales up the base model, and preprocesses LR images with degradation-robust encoder for the ControlNet, which improves general SR effects. The aforementioned methods focus on modifications of the control branch, while neglecting the generative potential of the main branch. With the emergence of DiT's brilliant text-to-image ability, the feasibility of the ControlNet paradigm on DiT-based SR modeling should be reconsidered.



==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_method.tex <==

\section{Method}
\label{sec:method}
In this section, we delve into the details of our Enhancing Anything Model (EAM). 
As shown in ~\cref{framework}, EAM consists of three parts: a new DiT-based architecture named $\Psi$-DIT, a new Progressive Masked Image Modeling Strategy in training, and a new pipeline to generate better prompts.
In the first section, we present an overview of our full Diffusion Image Transformer ($\Psi$-DiT) architecture, 
detailing the module design of the Subject-Sensitive Control Module (SSCM) and our strategy for weight initialization. 
In the second section, 
we delve into the Progressive Masked Image Modeling (MIM) Strategy that we have specifically tailored for the blind super-resolution task. 
Section 3 is dedicated to introducing our In-Context Learning (ICL)-based paradigm for Low-Resolution (LR) semantic extraction.
% As shown in ~\cref{framework}, 
\subsection{Overall Structure}

\input{figures/fDIT_note}

\paragraph{$\Psi$-DiT.}
The LR ControlNet~\cite{zhang2023addingconditionalcontroltexttoimage} module, initially introduced by DiffBIR~\cite{lin2023diffbir}, has been widely applied in the field of real-world super-resolution after inheritance and further improvement by PASD, SeeSR, and SUPIR~\cite{yang2023pixel, wu2024seesrsemanticsawarerealworldimage, yu2024scalingexcellencepracticingmodel}, and has been further adapted to the DiT series of models. However, we believe that the ControlNet architecture has significant limitations when used for real-world super-resolution tasks based on the DiT series models~\cite{esser2024scalingrectifiedflowtransformers, li2024hunyuanditpowerfulmultiresolutiondiffusion}. Firstly, it requires the replication of the entire base model's branches, which is costly in terms of training. Secondly, the direct addition of noisy latent and LR latent, two different modalities, limits the model's generative capabilities. To address the identified limitations, we introduce a novel architecture named $\Psi$-DiT. This architecture distinctively segregates the input modalities—text tokens, noisy latent tokens, and low-resolution (LR) tokens—on an architectural level. Each modality is processed by distinct DiT modules, with cross-modal interactions facilitated exclusively through attention modules. As depicted in ~\cref{content}, the original dual-stream MMDIT architecture, which was solely text-driven, has evolved into a triple-stream architecture. This new design is mirrored and controlled by both text and LR images. Simultaneously, to preserve the generative capabilities of the pre-trained T2I model to the fullest extent, we have chosen to freeze the weights of the text control branch inherited from the pre-trained T2I base model during training. This allows us to focus training on the newly integrated LR latent control branch. Ultimately, this approach offers two significant advantages. Firstly, compared to the full copy strategy of ControlNet, our $\Psi$-DiT architecture introduces only one additional branch, thereby minimizing the increase in new training parameters. Secondly, the LR latent control branch, which exerts conditional control solely through attention modules, is anticipated to maximize the utilization of the model's prior knowledge and mitigate the risk of degenerate overfitting.
\paragraph{separate stream control module.}
In the original MMDIT module, the noisy latent and text embeddings utilize distinct linear and multilayer perceptron (MLP) layers. During the attention calculation phase, the query (q), key (k), and value (v) vectors of the noisy latent and text embeddings are concatenated along the token dimension before performing the attention computation. Once the outputs are split, each is directed to their respective MLP modules via a linear layer.

As illustrated in ~\cref{content}., we have introduced a new stream-based separate conditional control module, termed the sscm, which builds upon the MMDIT framework. This sscm module takes as input the tokens from both the noisy latent branch and the low-resolution (LR) latent branch. In a manner akin to the MMDIT module, the qkv vectors of the noisy latent and LR latent are concatenated along the token dimension for attention calculation. Post-output splitting, the portion corresponding to the noisy latent is merged with the input at the noisy latent position of the MMDIT module through a linear layer. Concurrently, the output at the LR latent position is fed into the MLP module through a linear layer, acting as the input for subsequent processing blocks.
\paragraph{Weight initialization policy.}
In downstream tasks, weight initialization plays a pivotal role, influencing not only the model's convergence rate but also its ultimate generalization capabilities. Recognizing this, we have crafted specific weight initialization strategies aimed at bolstering the model's performance and efficiency. A key factor in the remarkable success of ControlNet was the incorporation of zero-conv, which substantially accelerated convergence. Building on this insight, we have integrated a zero-initialized layer in the final attention layer of our model. This addition ensures a seamless transition from text-to-image tasks to image-to-image tasks, leveraging the successful precedent set by zero-conv.

Naturally, we inherit the weights of the mirrored pre-trained model for the qkv of the noisy latent, as it aligns with our approach. However, for the weight initialization of the image control branch, we face a choice between two strategies. The first is to inherit the weights from the text control branch, which, like the image control branch, is a conditional branch. The second option is to adopt the weights from the noisy latent branch, which shares a similar modality.After careful consideration, we have chosen to initialize the weights of the LR latent branch by copying those of the noisy latent branch. This decision is rooted in the closer modality relationship between the LR latent and the noisy latent, making the transfer of weights more logical and beneficial for the model's performance.

\subsection{Progressive MIM Strategy}
% (can be moved to introduction parts if needed)
Masked Image Modeling (MIM) has been introduced to many high-level vision tasks.
It enables models to acquire a generic representation of images and 
thereby enhancing their generalization capabilities across a variety of tasks.
Masked Autoencoder (MAE)~\cite{he2021maskedautoencodersscalablevision} is a typical MIM approach, 
capable of reconstructing the entire image from masked, partial inputs.
Leveraging MIM, models can automatically infer and supplement missing information from even minimal input data. 
Building on this insight, we integrate MIM into our diffusion-based super-resolution network to enhance its generative capabilities.

However, the primary purpose of MIM in high-level vision tasks diverges from that in low-level vision tasks, 
making the direct application of MIM to low-level tasks sub-optimal.
In low-level vision, the typical goal is to enhance a low-quality image to achieve high-quality output. 
In contrast, MIM aims to generate a complete image from a masked input.
The degradation domains of MIM task are congruent, 
meaning that both the masked and restored images share similar levels of degradation or cleanliness.
Consequently, when adapting MIM to low-level visual tasks such as super-resolution, 
it is crucial to consider how to make the network aware of the degradation process.
This definitely raises the difficulties of the learning task for the network.
It is challenging for the network to hold a balance between its generative capabilities and the preservation of the original image information, 
and there is a significant risk that this imbalance could lead to a collapse.

Inspired by these insights, we have designed a novel \textbf{P}rogressive \textbf{M}asked Image Modeling \textbf{S}trategy (PMS) 
that leverages curriculum learning~\cite{wang2021surveycurriculumlearning} principles.
This strategy enables the model learning masked image super-resolution from more familiar to unfamiliar examples by controlling the mask ratio.
It smoothly transfer the network from a text-to-image(T2I) model to image-to-image(I2I) model.
We observed that PMS significantly enhances training stability and 
results in the generation of more realistic and detailed image features.

Specifically, given the mask ratio threshold $r_{min}$, and the total number of MIM training steps $t$, 
as well as the number of progressive steps $k$ and progressive clip $c$. 
We adjust the mask ratio based on the number of training steps $p$. 
When the number of training steps $p$ haven't reach $k$, the mask ratio will be random picked from a corresponding range.
Once the training steps $p$ is larger than $k$, the mask ratio will fixed to $r_{max}$ till the end of MIM training.
\begin{equation}
\begin{cases}
r = 1- ( 1 - r_{min}) \cdot (\lfloor \frac{p \cdot c}{k} \rfloor + \sigma) / c , & \text{if } p < k
 \\
r = r_{min}, & \text{if } p \geq k
\end{cases}
\end{equation}
Here, $\sigma \sim \mathcal N(0,1)$ is a random item. 
We use $t/2$ as a default value of $k$, and $s$  as a default value of $c$.

Compared with selecting random mask ratios throughout the training process, 
models using PMS are more likely to encounter image pairs with larger mask ratios at the beginning, 
aligning closely with the original T2I training paradigm. 
As the training progresses, the model gradually adapts to condition injections, 
it becomes more likely to encounter image pairs with a lower mask ratio. 
Then it allows for a deeper exploration of the model's generative capabilities based on reference images.

In addition, we use unmasked data pairs to perform SFT, 
which further strengthens the model's ability to remove degradation based on its generation capabilities.
Experiments have proven that using unmasked data to perform SFT can effectively improve pixel-level alignment capabilities. 
For specific experimental results, please refer to \cref{tab:pms_comp} and \cref{fig:ab2}.

\subsection{Subject-aware Prompts Generation}

When we see an image, our brain allocates different attention to different regions within the image. 
Typically, for images with a clear focal point, the brain tends to concentrate more on the content within the focal area 
before shifting attention to the non-focal regions. 
Conversely, for images with ambiguous or no focal points, such as wide-angle shots, 
the brain tends to distribute its attention more evenly across the entire image, focusing on the overall content and detail.

Building upon this observation, we have developed a description generation pipeline that 
leverages a state-of-the-art Vision-and-Language Model (VLM) to generate prompts for training. 
In this pipeline, the VLM first identifies the focal regions of an image. 
It then proceeds to describe these focal areas with as much detail as possible. 
For the non-focal regions, the VLM generates descriptions speculatively, based on the available visual cues. 
In cases of images with no clear focus, such as wide-angle shots, 
the VLM enhances its speculative descriptions to cover the entire image, ensuring a comprehensive narrative.

As show in ~\cref{framework}, we have select a collection of sample images that encompass both focused and non-focused areas. 
Utilizing in-context learning, we providing a set of ideal output results at beginning. 
These samples, along with their corresponding ideal results, serve as the example inputs for our VLM model.
Then the VLM can annotate the next input image with previous given examples.

The prompts generated through this pipeline are more sensitive to the focal points of the images compared to simply describe them. 
This approach yields richer details and incorporates more speculative content, which significantly enhances the model's generation capabilities. 
For further experimental validation and results, please refer next section.


==> sec/4_exp.tex <==
\section{Experiments}
\label{exp}
% \input{table/tab1}
\input{figures/maincompare}
\input{figures/real_compare}
\subsection{Experimental Settings}
\paragraph{Training Datasets.}
We train EAM on LSDIR~\cite{li2023lsdir}, DIV2K~\cite{timofte2017div2k}, Flickr2K ~\cite{agustsson2017flicker2k}, OST~\cite{wang2018ost}, and the first 10K face images
from FFHQ~\cite{ffhq}. To generate training pairs of low-resolution (LR) and high-resolution (HR) images, we employed the degradation pipeline from Real-ESRGAN~\cite{wang2021real}. 
\paragraph{Test Datasets.}
In order to compare the performance of different real-world superseparation methods more comprehensively, we use synthetic data and real-world data as test sets to evaluate the metrics.
1) First, we use 100 verification set images of DIV2K~\cite{timofte2017div2k}, resize the short edge to 1024, and then crop the center through the degenerate pipeline that is consistent with the training to generate pairs of LR-HR data pairs. We named this dataset DIV2K-VAL.
2) Use the real world dataset, realphoto60, and all resize to 1024 to inference collected in SUPIR~\cite{Fanghua2024supir}.
3) Adhering to the protocols of the latest blind image super-resolution competition, we have adopted the real-world test set from the final stage of the NTIRE 2024 RAM competition~\cite{RAIM} as our benchmark. This set encompasses 50 real-life images captured on actual phones, ensuring a practical and accurate assessment of our model's capabilities.
\paragraph{Implementation Details.}
We used SD3-medium~\cite{esser2024scalingrectifiedflowtransformers} as our pre-trained T2I model. Our Enhancing Anything Model (EAM) utilizes the Adam optimizer for training, which is conducted over 30,000 iterations. The entire experiment was conducted using 1024-resolution images, leveraging 32 NVIDIA GeForce RTX A100 graphics cards.
\subsection{Comparison with Existing Methods}
\paragraph{Quantitative Comparisons.}
As illustrated in \cref{tab:metric_tab}, our methodology effectively addresses a wide range of image degradations. In our quantitative evaluation, we employ Real-ESRGAN's degradation protocols to rigorously benchmark our approach against state-of-the-art algorithms that share similar objectives, including StableSR~\cite{wang2023exploiting}, DiffBIR~\cite{lin2023diffbir}, PASD~\cite{yang2023pixel}, SeeSR~\cite{wu2024seesrsemanticsawarerealworldimage}, and SUPIR~\cite{yu2024scalingexcellencepracticingmodel}.

Our evaluation encompasses three distinct datasets: DIV2K, RealWorld60, and RAM50. RealWorld60 is sourced from the SUPIR dataset~\cite{Fanghua2024supir}, while RAM50 is drawn from the NTIRE2024 challenge~\cite{RAIM}. To streamline the metric computation process, we extract a central square crop from the output images. The evaluation metrics are a comprehensive set of full-reference metrics, comprising PSNR, SSIM, and LPIPS, alongside no-reference metrics such as ManIQA~\cite{yang2022maniqamultidimensionattentionnetwork}, ClipIQA~\cite{wang2022exploringclipassessinglook}, and MUSIQ~\cite{ke2021musiqmultiscaleimagequality}. Owing to the unavailability of ground truth images in RealWorld60 and RAM50, our comparative analysis relies exclusively on no-reference metrics. 

Our method exhibits satisfactory performance in full-reference metrics on the DIV2K dataset, suggesting a considerable level of fidelity. Additionally, it shows strong competitiveness in no-reference metrics across all three datasets, with only a few metrics slightly underperforming compared to DiffBIR.

\paragraph{Qualitative Comparisons.} 

In comparison to the current state-of-the-art models such as SUPIR, our model achieves a more favorable balance between fidelity and generativity. The EAM structure, equipped with multiple advanced techniques, excels in regions with clear semantics, such as hair, vegetation, and architectural structures.

As shown in the accompanying Fig. \ref{fig1:main_visual}, our model demonstrates superior realism and clarity in animal fur, surpassing other methods. It also exhibits good generative capabilities on medium to small faces without any facial distortion or noticeable facial defects.

As depicted in Fig. \ref{RealWorld Compare}, leveraging the powerful prior capabilities of SD3, our model shows significant competitiveness in terms of scene authenticity and detail. Moreover, it possesses an extremely strong generalization ability, truly achieving super-resolution for all things. Fig. \ref{ab1} further corroborate the model's advanced super-resolution capabilities, with no apparent weaknesses in its performance.

%\paragraph{User Study.} 



\subsection{Ablation Study}
\label{exp_abl}
\paragraph{Compare with ControlNet.}
\input{table/table_psi}
\input{table/table_init}
\input{figures/ab1}
Although the DiT architecture augmented with a ControlNet~\cite{zhang2023addingconditionalcontroltexttoimage} branch achieves commendable results after 80k iterations, our proposed $\Psi$-DiT achieves convergence with only 30k iterations.
$\Psi$-DiT, based on the MAE training paradigm, conserves training costs and enhances convergence speed.
The conditional input branch, token-based, offers greater flexibility and is more compatible with the MAE training approach.

As shown in Table ~\ref{tab:psi}, on the DIV2K dataset, $\Psi$-DiT surpasses DiT-ControlNet in ClipIQA and MUSIQ metrics. On the open-source dataset NTIRE2024 RAM50, $\Psi$-DiT leads across ManIQA, ClipIQA, and MUSIQ metrics, demonstrating $\Psi$-DiT's robust generative capabilities and excellent generalization in diverse scenarios.

Furthermore, as indicated in Table \ref{tab:init}, our zero initial strategy ensures the maximization of the inherent generative potential of the original SD3, preserving the information contained in the parameters of the original DiT structure from the outset of training.
We have meticulously selected the parameters for the noisy latent branch (NLB) to initialize the conditional branch.
Compared to initialization with a text embedding branch (TEB), noisy latent branch initialization better adapts the conditional branch to LR image tokens.

\paragraph{Progressive MIM Strategy.} 
\input{figures/ab2}
To better migrate Masked Image Modeling (MIM) into our model, 
we conducted experiments with various mask ratios to comprehensively assess their influence on model performance.
As illustrated in Table ~\ref{tab:pms_comp}, comparing a fixed mask ratios of 0.5 and 0.75, 
we observe that employing a mask ratio that is too low diminishes the model's generative capacity, 
consequently leading to a decline in metrics.
We then explored several approaches to increasing the mask ratio. 
One method involved maintaining a high mask ratio of 0.85, another utilized a random mask ratio ranging from 0.75 to 1.0, 
and the third employed our proposed Progressive Masked Image Modeling (PMS) strategy. 
Our analysis revealed that, compared to the default mask ratio of 0.75, 
PMS not only achieved superior performance metrics but also reduced the training costs for the network. 
This result further substantiates the advantages of PMS in transitioning from T2I models to I2I models.
\input{table/table_PMS}

\paragraph{Subject-aware Prompts.} 
The efficacy of subject-aware prompts is shown in Table ~\ref{tab:prompts_comp}. 
The table indicates that if the model inference uses only prompts collected by the subject-aware method, its performance is sub-optimal. 
However, by incorporating these subject-aware prompts during the training phase, 
the model can fully leverage its subject-aware capabilities, thereby enhancing the final result.
\input{table/table_prompts}


==> sec/5_col.tex <==
\section{Conclusion}

With the advent of the Diffusion Image Transformer (DiT) as a formidable diffusion network,
the emergence of DiT-based super-resolution (SR) models is imminent. 
It is anticipated that within these DiT-based SR networks, 
the constraints of the Controlnet will emerge as a bottleneck, 
hindering the achievement of exceptional SR performance. 
To counteract this limitation, we introduce in Enhancing Anything Model (EAM), a novel DiT-based architecture designed for blind image super-resolution. 
Leveraging a pre-trained text-to-image DiT, we construct a triple-flow DIT block, 
denoted as $\Psi$-DiT, which integrates the noise latent variable with the text embedding and low-resolution (LR) latent variable to enhance attention mechanisms. 
Our ablation studies demonstrate that these novelty blocks outperform the conventional Controlnet. 
Furthermore, during training, we incorporate Progressive MIM Strategy to enhance the generative capacity and robustness of our model. 
Additionally, we employ a new subject-aware prompt generation pipeline to supply more insights to the model through in-context learning, which significantly benefits the SR results. 
Extensive experiments confirm that our model excels current SR methodologies on real-world datasets.

==> table/tab1.tex <==
\begin{table*}[t]

 \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
 \begin{center}
 \scalebox{0.85}{
% \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|cccccc}
                \hline Datasets & Metrics & \makecell[c]{StableSR} & \makecell[c]{DiffBIR} & \makecell[c]{PASD} & \makecell[c]{SeeSR} & \makecell[c]{SUPIR} &    \makecell[c]{EAM} \\
                \hline \multirow{6}{*}{\makecell[c]{DIV2K-Val}} & PSNR $\uparrow$ & \rf{21.07} & 20.94 & 20.95 & \bd{21.02} & 19.93 & 19.87 \\
                 & SSIM $\uparrow$ & \rf{0.5687} & 0.5398 & 0.5626 & \bd{0.5662} & 0.5189 & 0.5225  \\
                 & LPIPS $\downarrow$ & 0.3767 & 0.3728 & 0.3821 & \bd{0.3321} & 0.3655 & \rf{0.3318} \\
                 & ManIQA $\uparrow$ & 0.5396 & \bd{0.6085} & 0.5511 & 0.6215 & \bd{0.0.6321} & \rf{0.6601} \\
                & CLIP-IQA $\uparrow$ & 0.5357 & \rf{0.7258} & 0.6158 & 0.7092 & 0.6252 & \bd{0.7150} \\
                & MUSIQ $\uparrow$ & 61.20 & 70.89 & 69.12 & \bd{72.32} & 70.88 & \rf{73.95} \\
                \hline \multirow{3}{*}{\makecell[c]{RealWorld60}}
                 & ManIQA $\uparrow$ & 0.5003 & \bd{0.6087} & 0.5232 & 0.6067 & 0.6044 & \rf{0.6333} \\
                 & CLIP-IQA $\uparrow$ & 0.5278 & \rf{0.7729} & 0.6143 & \bd{0.7379} & 0.6561 & 0.715 \\
                & MUSIQ $\uparrow$ & 54.59 & \bd{69.84} & 63.14 & \bd{71.46} & 70.47 & \rf{73.95} \\
                \hline \multirow{3}{*}{\makecell[c]{NTIRE2024-RAM50}}
                 & ManIQA $\uparrow$ & \bd{0.6986} & 0.6482 & 0.6497 & 0.6639 & 0.6531 & \rf{0.7135} \\
                & CLIP-IQA $\uparrow$ & 0.6857 & \rf{0.7034} & 0.6644 & 0.6886 & 0.5199 &  \bd{0.7027}\\
                & MUSIQ $\uparrow$ & \bd{72.98} & \bd{71.87} & 72.14 & 72.79 & 67.36 & \rf{73.56} \\
                \hline
  \end{tabular}
}
\caption{Quantitative comparison with state-of-the-art methods on both synthetic and real-world benchmarks. \rf{Red} and \bd{blue} colors represent the best and second best performance, respectively.}
 \end{center}
 \vspace{-0.25cm}
\label{tab:metric_tab}
\end{table*}

==> table/table_PMS.tex <==
\begin{table}[h]
    \centering
    \hspace{-2.5mm}
    \scalebox{1}{
    \begin{tabular}{ccccc}
    \toprule
        Mask Strategy  & ManIQA & ClipIQA & MUSIQ \\
        \midrule
        No Mask &  0.6584 & 0.6813 & 73.14\\
        Fix 0.50 & 0.7051 & 0.6826 & 73.08\\
        Fix 0.75 & 0.6897 & 0.6916 & 73.20\\
        Fix 0.85 & 0.7048 & 0.6916 & 72.32\\
        Random 0.75$\sim$1.00 & 0.7072 & 0.6953 & \textbf{73.60}\\
        PMS (ours) & \textbf{0.7077} & \textbf{0.6984} & 73.44\\
        \bottomrule
    \end{tabular}}
    \vspace{-3mm}
    \caption{Comparison on different MIM strategy on NTIRE2024-RAM50. \textbf{Bold} represent the best performance.}
    \label{tab:pms_comp}
    \vspace{-2mm}
\end{table}




==> table/table_init.tex <==


\begin{table}[h]
    \centering
    \hspace{-2.5mm}
    \scalebox{0.5}{
    \begin{tabular}{ccccccccc}
    \toprule
		\textbf{zero initial} & \textbf{TEB initial} & \textbf{NLB initial} & \textbf{PSNR} & \textbf{SSIM} & \textbf{LPIPS} & \textbf{ManIQA} & \textbf{ClipIQA} & \textbf{MUSIQ} \\ \midrule
		$\times$ & $\times$ & $\times$ & 19.66 & 0.5089 & 0.3669 & 0.6331 & 0.6816 & 73.18 \\
		\checkmark & $\times$ & $\times$ & 19.61 & 0.5117 & 0.342 & 0.6362 & 0.6899 & 73.24 \\
		\checkmark & \checkmark & $\times$ & 19.87 & 0.5183 & 0.3276 & 0.6511 & 0.7023 & 73.39 \\
		\checkmark & $\times$ & \checkmark & 19.75 & 0.5197 & 0.3329 & 0.6584 & 0.7142 & 73.86 \\ 
  \bottomrule
    \end{tabular}}
    \vspace{-3mm}
    \caption{Methods for Initializing the Conditional Branch, where TEB initial refers to the initialization from the text embedding branch, and NLB initial indicates the initialization from the noisy latent branch
    }
    \label{tab:init}
    \vspace{-2mm}
\end{table}


==> table/table_prompts.tex <==
\begin{table}[h]
    \centering
    \hspace{-2.5mm}
    \scalebox{1}{
    \begin{tabular}{ccccc}
    \toprule
        Training & Testing  & ManIQA & ClipIQA & MUSIQ \\
        \midrule
        DA & DA &  0.6326 & 0.7333 & 73.13\\
        DA & SA & 0.6301   & 0.7326 & 72.69  \\
        SA & SA & \textbf{0.6416} & \textbf{0.7652} & \textbf{73.95}\\
        \bottomrule
    \end{tabular}}
    \vspace{-3mm}
    \caption{Comparison on different prompts training \& testing strategy on RealPhoto60. \textbf{Bold} represent the best performance.DA refers to detail-aware prompts, which is the traditional prompts generation method. SA refers to subject-aware prompts, which applied our new pipeline of prompts generation. }
    \label{tab:prompts_comp}
    \vspace{-2mm}
\end{table}


==> table/table_psi.tex <==




\begin{table}[t]
    \centering
    \hspace{-2.5mm}
    \scalebox{0.6}{
    \begin{tabular}{ccccccccc}
    \toprule
		\textbf{architecture} & \textbf{best iters} & \textbf{PSNR} & \textbf{SSIM} & \textbf{LPIPS} & \textbf{ManIQA} & \textbf{ClipIQA} & \textbf{MUSIQ} \\ \midrule
		DiT-controlnet & 80k & 20.07 & 0.5291 & 0.318 & 0.6502 & 0.703 & 73.25 \\
		$\Psi$-DiT & 30k & 19.75 & 0.5197 & 0.3329 & 0.6584 & 0.7142 & 73.86  \\ 
  \bottomrule
    \end{tabular}}
    \vspace{-3mm}
    \caption{
    Ablation on the key architecture.
    }
    \label{tab:psi}
    \vspace{-2mm}
\end{table}

